Goodbye to Chi-by-Eye: A Bayesian Analysis of Photometric Binaries in Six Open Clusters

We present a robust methodology for identifying photometric binaries in star clusters. Using Gaia DR3, Pan-STARRS and 2MASS data, we self-consistently define the cluster parameters and binary demographics for the open clusters (OCs) NGC 2168 (M35), NGC 7789, NGC 6819, NGC 2682 (M67), NGC 188, and NGC 6791. These clusters span in age from ~200 Myr (NGC 2168) to more than ~8 Gyr (NGC 6791) and have all been extensively studied in the literature. We use the Bayesian Analysis of Stellar Evolution software suite (BASE-9) to derive the age, distance, reddening, metallicity, binary fraction, and binary mass-ratio posterior distributions for each cluster. We perform a careful analysis of our completeness and also compare our results to previous spectroscopic surveys. For our sample of main-sequence stars with masses between 0.6 - 1 M_Sun, we find that these OCs have similar binary fractions that are also broadly consistent with the field multiplicity fraction. Within the clusters, the binary fraction increases dramatically toward the cluster centers, likely a result of mass segregation. Furthermore nearly all clusters show evidence of mass segregation within the single and binary populations, respectively. The OC binary fraction increases significantly with cluster age in our sample, possibly due to a combination of mass-segregation and cluster dissolution processes. We also find a hint of an anti-correlation between binary fraction and cluster central density as well as total cluster mass, possibly due to an increasing frequency of higher energy close stellar encounters that inhibit long-period binary survival and/or formation.

==> old_response.tex <==
We thank the referee very much for the timely report and the useful comments that have improved the manuscript.  We have added our responses to the referee in this text as well as in the attached PDF.  New additions to the manuscript are shown in red text.

--------------------------------------------------------------
Reviewer:
I have reviewed the manuscript written by Childs et al. entitled "Goodbye to Chi-by-Eye: A Bayesian Analysis of Photometric Binaries in Six Open Clusters". 
The authors applied the latest version of Bayesian Analysis of Stellar Evolution code (BASE-9) on the publicly available data such as the Gaia DR3, to "self-consistently" derive the age, distance, reddening, metallicity, binary fraction, and binary mass-ratio for six galactic open clusters whose ages range from 200 Myr to 8 Gyr. As the authors mentioned, this is a methodology paper aiming to set up an efficient and "self-consistent" way to analyze a large set of multiband photometric data for their future works. Therefore the results from their Bayesian analysis might not be ground-breaking or brand new findings for these well-studied six open cluster samples. Among the characteristic physical parameters of the Galactic open clusters, the authors focused on the parameters of photometric binary populations such as binary fraction and binary mass-ratio that require time-consuming processes and difficult to obtain 'complete' values from spectroscopic observations. 

The Bayesian approach suggested by the authors for investigating the photometric binary populations in the Galactic open clusters could be a very efficient alternative tool as compared to traditional methods (e.g. isochrone fitting by eye using independent measurement of distance). However I do have a couple of major concerns on the current form of the manuscript. I must say a significant revision is needed for publication: 

First, about the usage of Pan-STARRs and 2MASS data. 
The authors claim that they used Pan-STARRs and 2MASS data along with Gaia DR3 to characterize individual stellar masses, binary mass ratio, and photometric membership probabilities for each target open cluster (Page 3, line 179-188). However I cannot find any further detailed explanations, analysis, figures on how these Pan-STARRs and 2MASS data were used in their Bayesian analysis throughout the manuscript. I think this should be a significant issue in this manuscript because the authors insisted that their study is distinguished from the previous studies (Cordoni et al. 2023; Jadhav et al. 2021; Cohen et al. 2020) by incorporating Pan-STARRs and 2MASS, and using the latest BASE-9 code. The authors should present their answers to the following questions in order to justify their claim on the usage of Pan-STARRs and 2MASS data in the Bayesian analysis. 

RESPONSE:  BASE-9 uses photometric data from all three surveys when using MCMC to fit isochrones.  While we originally presented only CMDs for the Gaia filters, BASE-9 considers all filter combinations in each survey when fitting isochrones.  We have also added the extra CMDs to the Appendix.  We have added clarification of this to the beginning of Section 2.

Q. How did the authors figure out the cross-matching issue between the optical Gaia data and NIR 2MASS data especially for the open clusters with dense cores such as NGC2682, NGC6791, and NGC6819? 

RESPONSE: We use Gaia's pre-computed cross matches for both Pan-STARRS and 2MASS.  We have added this detail to the beginning of Section 2.

Q. Are those mass-limited main-sequence star (ML-MS) samples also well recovered in the 2MASS color-magnitude diagrams? 

RESPONSE: Yes.  Because BASE-9 considers all photometry sets simultaneously, the same stars are recovered in each survey.

Q. The authors mentioned "differential reddening" in section 2.3. Using 2MASS CMDs should have advantages over the optical Gaia data to deal with the differential reddening issues. Have the authors tried to use 2MASS CMDs? 

RESPONSE:  Yes, BASE-9 also considers the CMDs from 2MASS. 

Second, section 4.6 "Binary mass-ratio distributions" is totally missing so that I cannot judge if this manuscript is publicable or not. 

RESPONSE:  The placement of Section 4.6 was a typo.  We have corrected this so that the two paragraphs initially found about Section 4.6 are now included in Section 4.6.

I outline several comments/questions/concerns in each section on the PDF file. Please place your cursor on the sentences with red underline using Acrobat Reader. You can see my comments/questions.

RESPONSE:  We have responded to all of the additional comments in the attached PDf.

Data/Software Review :
One of our data editors has reviewed your initial manuscript submission and has the following suggestion(s) to help improve the data, software citation and/or overall content. Please treat this as you would a reviewer's comments and respond accordingly in your report to the science editor. Questions can be sent directly to the data editors at data-editors@aas.org

I. In addition the visualization tools provided by the "Open Cluster Binary Explorer" we strongly encourage the authors to deposit the final catalogs in a machine-readable format into a DOI-issuing repository and include the resulting DOI in the revised manuscript. Our current tutorial for using Repositories is found at the following URL, though note that an institutional repository can also work for this purpose. Based on my use of the "Open Cluster Binary Explorer" there may be many different kinds of derivative files, e.g., summary stats for clusters as well as posteriors for individual objects. As such the description supplied for the DOI-deposited material should be complete, covering how a reader might use each data type. 

RESPONSE: We have published our data sets on Zenodo: DOI 10.5281/zenodo.10080682

II. It may seem unnecessary, but we think it important to cite the specific sources for the data used. For example, there are at least three ways to obtain Gaia DR3 and the specific provenance matters (Gaia/ESA supplied [https://doi.org/10.5270/esa-qa4lep3]; Vizier [https://doi.org/10.26093/cds/vizier.1355]; and IRSA [https://doi.org/10.26131/IRSA544]). You can mention and cite the specific dataset DOIs used for Gaia as well as Pan-STARRS and 2MASS if possible.

RESPONSE:  We have added the Gaia DR3 DOI, and the standard acknowledgements for the Pan-STARRS and 2MASS surveys in the "Facilities" section.  Additionally, we have included all of the relevant citations for each of these surveys in the text.



==> response.tex <==
We thank the referee very much for the timely report and the useful comments that have improved the manuscript.  We have added our responses to the referee in this text.  New additions to the manuscript are shown in red text.

--------------------------------------------------------------

Reviewer:
I have read the revised manuscript and find that the authors have made a significant improvement by including important plots (i.e. PanSTARRS & 2MASS CMDs) that I requested in my first review. However there still remains an issue that I would like to see to be cleared up before publication. 

Overall, in terms of the methodology and analysis process that the authors provided, I don't have any significant complaints. However, what I still want to point out is about "coherency" in the authors' claims (or arguments) on "the robustness of their methodology" in the following part: 

** On the usage of 2MASS CMDs
In page 2, the authors give a general introduction to "photometric binary studies" saying that "This method requires high precision photometry and a careful isochrone fit to the cluster members." (line 129-131). Indeed the authors follow this principle and decide not to apply reddening corrections on the collected photometric data (Gaia DR3 + PanSTARRS + 2MASS) for NGC6819 and NGC7789 (line 342-349 in page 5) because the reddening corrections introduce photometric uncertainties too large for BASE-9 to derive precise cluster parameters. If this is the case, what about the 2MASS photometry of NGC188 and NGC6791? Looking at the 2MASS CMDs (Figure 12 in page 23) of NGC188, NGC6791, NGC6819, and NGC7789, I must say that the uncertainty level of the 2MASS photometry itself for the cross-matched members in these 4 OCs seems to be too large for any kind of photometric analysis. I don't think the 2MASS data of these 4 OCs are appropriate to the BASE-9 analysis, and they should be opted out from the analysis of this study. However, if the authors still want to include the 2MASS data for these 4 OCs in their analysis, the authors should come up with a better color combination (e.g. Gbp - K or g - K) including 2MASS bands just like Cohen et al.(2020) did in their study (i.e. V vs (B-K) CMD), otherwise the authors must show a quantitative analysis where/how much improvement can be achieved by including the 2MASS data in their analysis. This can be done relatively easily - Since the main results of this study from the BASE-9 analysis are presented from Figure 6 to Figure 11, what would be the results if the 2MASS data were not included in the BASE-9 analysis?

RESPONSE:  When reddening corrections are applied, the uncertainties on all three data sets are increased accordingly.  The 2MASS data is used complimentary to Gaia and Pan-STARRS data, and the large uncertainities on 2MASS data do not affect the relatively small uncertainties on Pan-STARSS and Gaia data.  Conceptually, BASE-9 will never do "worse" by adding more data, assuming the errors are appropriate.  A dataset with large errors (like the fainter stars in 2MASS data) won't be as constraining on model parameters as a dataset with smaller errors.  Therefore we expect that the brighter stars in 2MASS data will provide useful constraints on the cluster parameters, while the fainter 2MASS stars will be less useful.  To better understand how 2MASS data affects our results we have rerun our pipeline for the six clusters, omitting 2MASS photometry.  We found that when fitting the isochrone, the posterior distributions (shown in Figure 2) are similar, indicating that the sampling is largely determined by the more precise and numerous Gaia and Pan-STARRS photometry.  When determining cluster membership and stellar binarity using photometry without 2MASS, BASE-9 finds at least 98\% of members from our standard pipeline but finds only 75\%-95\% the number of binaries.  This is because 2MASS extends the SEDs and can place tighter constraints on stellar binarity for the brighter stars (with smaller 2MASS photometric uncertainties), especially for low q binaries which may otherwise classified as single stars by BASE-9.  We have added these points to Section 3 and updated the color combinations for the 2MASS CMDs in Figure 12 and Figure 15 as the referee suggests.  

Data/Software Review :
One of our data editors has reviewed your initial manuscript submission and has the following suggestion(s) to help improve the data, software citation and/or overall content. Please treat this as you would a reviewer's comments and respond accordingly in your report to the science editor. Questions can be sent directly to the data editors at data-editors@aas.org

I. In addition the visualization tools provided by the "Open Cluster Binary Explorer" we strongly encourage the authors to deposit the final catalogs in a machine-readable format into a DOI-issuing repository and include the resulting DOI in the revised manuscript. Our current tutorial for using Repositories is found at the following URL, though note that an institutional repository can also work for this purpose. Based on my use of the "Open Cluster Binary Explorer" there may be many different kinds of derivative files, e.g., summary stats for clusters as well as posteriors for individual objects. As such the description supplied for the DOI-deposited material should be complete, covering how a reader might use each data type. 

RESPONSE: We have published our data sets at https://doi.org/10.5281/zenodo.10080762

II. It may seem unnecessary, but we think it important to cite the specific sources for the data used. For example, there are at least three ways to obtain Gaia DR3 and the specific provenance matters (Gaia/ESA supplied [https://doi.org/10.5270/esa-qa4lep3]; Vizier [https://doi.org/10.26093/cds/vizier.1355]; and IRSA [https://doi.org/10.26131/IRSA544]). You can mention and cite the specific dataset DOIs used for Gaia as well as Pan-STARRS and 2MASS if possible.

RESPONSE:  We have added the Gaia DR3 DOI, and the standard acknowledgements for the Pan-STARRS and 2MASS surveys in the "Facilities" section.  Additionally, we have included all of the relevant citations for each of these surveys in the text.
